Total Variation Regularized Tensor-on-scalar Regression

In this paper, we propose Total Variation Regularized Tensor-on-scalar Regression(TVTR), a novel method for estimating the association between a tensor outcome (a one dimensional or multidimensional array) and scalar predictors. While the statistical developments proposed here were motivated by the brain mapping and activity tracking, the methodology is designed and presented in generality and is applicable to many other areas of scientific research. The estimator is the solution of a penalized regression problem where the objective is the sum of square error plus a total variation (TV) regularization on the predicted mean across all subjects. We propose an algorithm for the parameter estimation, which is efficient and scalable in distributed computing platform. Proof of the algorithm convergence is provided and the statistical consistency of the estimator is presented via an oracle inequality. We presented 1D and 2D simulation results, and demonstrate that TVTR outperforms existing methods in most cases. We also demonstrate the general applicability of the method by two real data examples including the analysis of the 1D accelerometry subsample of a large community-based study for mood disorders and the analysis of the 3D MRI data from the attention deficient/hyperactive deficient (ADHD) 200 consortium.

==> convergence_bl.tex <==
\subsection{Algorithm}
\label{sec:algorithm}
Our goal is to estimate the multi-dimensional coefficients $\Gamma$ in the objective function~\eqref{eq:obj}. Although it is a convex function, the non-smoothness of the total variation regularization makes traditional algorithms suffer from slow convergence. 
In many applications, the optimization problem involves
a large number of variables, and cannot be efficiently
handled by generic optimization solvers. 

Instead, we propose to use the Alternating Direction Method of Multipliers (ADMM).
ADMM was originally introduced by~\cite{glowinski1975approximation,gabay1976dual} and has been frequently used in distributed settings (see~\cite{boyd2011distributed} for an overview). The idea of using ADMM to solve total variation regularized problems were first derived by \citet{wahlberg2012admm}, which introduced an efficient and scalable optimization algorithm for problems satisfying  a {\it TV-separability condition}.  The condition requires the cost function is the sum of two terms, one that is separable in the variable blocks, and a second that is separable in the difference between consecutive variable blocks. In each iteration of our method, the first step involves separately optimizing over each variable block, which can be carried out in parallel.
The second step is not separable in the variables, but can be carried out by applying ADMM to $L_1$ mean filtering very efficiently. 
This algorithm has been successfully applied to fused lasso and total variation denoising problems and exhibited competitive performance. It is also very easy to extend to distributed computing setting. %In this paper, we will focus on the single machine setting, and leave the parallelization for future work.

%Developed in the 1970s, ADMM bears close relation to many other optimization algorithms including Bregman iterative algorithms for $\ell_1$ problems, Douglas-Rachford splitting~\citep{eckstein1992douglas}, and proximal point methods; \citep{eckstein1992douglas}. 
%ADMM has been applied in many areas, including image and signal processing, as well as large-scale problems in statistics and machine learning (see e.g. \cite{boyd2011distributed}). It is suitable for distributed computing and is first used to solve total variation denoising problem in \citet{wahlberg2012admm}.
%We will also show that, combined with recent advances in graph fused lasso solvers, the algorithm converge to its global optimal. 

To make our problem satisfy the above {\it TV-separability condition}, we consider a reformulation of the original problem. Define $\theta=X\Gamma\in \bR^{n M}$, the problem is equivalent to,
\beq{
\bsplt{
\min_\theta \quad & \frac{1}{2}\| \ttvec(Y^T) -\theta\|^2_F +\lambda \| D_v^T\theta \|_{\ell_1};\\
\textrm{s.t.} \quad & (I-H_v)\theta=0.
}
\label{eq:cons_opt}\tag{CP}
}
The solution of \eqref{eq:obj} and that of \eqref{eq:cons_opt} have the following relationship.
%Our proposed algorithm is firstly inspired by the observation that the original problem \ref{eq:obj} is equivalent to the total variation denoising problem with the constraint that the solution signal can be written as the vectorization of the product of design matrix $X$ and some $\Gamma$. In other words, the solution signal belongs to the extended span of the design matrix $X$, or the projection to the orthogonal space equals to 0, $H_v\theta =0$. 
\begin{lemma}
\label{lem:theta2gamma}
Let $\that$ be the optimal solution of \eqref{eq:cons_opt}, and $\hat{\Gamma}$ be the optimal solution of \eqref{eq:obj}. If rank($X)=p$, then 
$
\hat{\Gamma}=(X^TX)^{-1}X^T \text{mat}(\that)_{n\times M}
$.
\end{lemma}
%{\color{red}The proof follows from a transformation of variable and can be found in supplementary materials.}

% ADMM
Now to solve \eqref{eq:cons_opt}, we introduce two auxiliary variables and write the original problem in the following form.
\ba{
\min & \quad \frac{1}{2}\|y-\theta\|^2+\delta((I-H_v)\eta=0)+\lambda \|D_v^T\mu\|_{\ell_1} \nonumber \\
s.t. & \quad \theta=\mu, \theta=\eta \label{eq:augmented_admm}
}
where $\delta(\cdot)$ is the characteristic function, which takes 0 if the condition in the parenthesis is satisfied and infinity otherwise. %By separating the least square term, the regularization term and the constraint term, we now use the Alternating Direction Method of Multiplier (ADMM) to solve it. 
The objective function is separable for $\theta, \eta$ and $\mu$, we solve it with the Alternating Direction Method of Multiplier (ADMM), which is summarized in Algorithm~\ref{alg:palm}.
\begin{algorithm}[h]
\caption{ADMM for Total Variation Regularized Tensor-on-scalar Regression}
\label{alg:alm}
\begin{algorithmic}[1]
\STATE {\bf Input}: Design matrix $X$, Images $Y$, %an off-the-shell Graph Fused Lasso solver (GFL); 
tuning parameter $\rho$, error tolerance $tol$.
\STATE Initialize  $\theta^{(0)}, \mu^{(0)}, \eta^{(0)}$ randomly; $U^{(0)}=V^{(0)}=\bm{0}_{nM}$; $k=0$; 
\WHILE{not converge}
\STATE $\theta^{(k+1)}=(\textrm{vec} (Y)+\rho(\eta^{(k)}-U^{(k)}+\mu^{(k)}-V^{(k)}))/(2\rho+1)$;
\STATE $\eta^{(k+1)}= H_v(\theta^{(k+1)}+U^{(k)})$;
\STATE $\mu^{(k+1)} = \arg\min_\mu \lambda\|D_v^T\mu^{(k)}\|_{\ell_1}+\frac{\rho}{2} \|\theta^{(k+1)} +V^{(k)}-\mu^{(k)}\|_F^2$;
\STATE $U^{(k+1)} = U^{(k)} +\theta^{(k+1)} -\eta^{(k+1)}$;
\STATE $V^{(k+1)} = V^{(k)}+\theta^{(k+1)} - \mu^{(k+1)}$;
\STATE $k=k+1$;
%\STATE converge {\bf if} $\max\{ | obj(\theta^{(k+1)}) - obj(\theta^{(k)})|, \|H_v\theta^{(k+1)}\|_F\} < tol$.
\STATE converge {\bf if} $\max\{ \|\theta^{(k+1)}) - \theta^{(k)})\|_F/\|\theta^{(k)})\|_F, \|H_v\theta^{(k+1)}\|_F\} < tol$.
\ENDWHILE
\STATE {\bf Output}: $\Gamma=(X^TX)^{-1}X^T\text{mat}(\theta^{(k+1)})_{n\times M}$;
\end{algorithmic}
\label{alg:palm}
\end{algorithm}


In Algorithm~\ref{alg:palm}, line 4-6 are the primal variable updates and line 7-8 are the dual variable updates. It is common practice to set $\rho=1$. The update of $\theta$ in line 4 and projection step in line 5 both have analytical form and only consist of matrix multiplication. The computational bottleneck is the subproblem in line 6, which can be recognized as a graph fused lasso (GFL) problem that takes observation $\theta_{k+1}+V_k$, regularization parameter $\lambda/\rho$, and graph incidence matrix $D_v^T$.
GFL is a generalization of fused lasso. It penalizes the first differences of the signal across edges and can be efficiently solved with many off-the-shell GFL solvers. Below we highlight several solvers for GFL, and compare their efficiency under different assumptions.
%It is worthing noting that in each subproblem, one basically solves a standard GFL problem. 

When the graph is a chain graph, the GFL reduces to a 1D fused lasso problem, and can be solved in $O(n)$ time, by, for example, the ``taut string" algorithm derived by \cite{davies2001local} and the dynamic programming based algorithm by \cite{johnson2013dynamic}. These methods are fast in practice. 
For 2D cases, \cite{kolmogorov2016total} generalizes the dynamic programming idea to solve the fused lasso problem on a tree in $O(n\log n)$ time. \cite{barbero2014modular} uses operator splitting techniques like Douglas-Rachford splitting and extends fast 1D fused lasso optimizers to work over grid graphs. Over general graphs structure, numerous algorithms have been proposed in recent years: \cite{chambolle2009total} described a direct algorithm based on a reduction to parametric max flow programming; \cite{chambolle2011first} described what can be seen as a kind of preconditioned ADMM-style algorithm; \cite{kovac2011nonparametric} described an active set approach; \cite{landrieu2016cut} derived a method based on graph cuts. In our experiments, we use the one proposed in \cite{tansey2015fast} which leverages fast 1D fused lasso solvers in an ADMM decomposition over trails of the graph. 
%{\color{red}
One can choose the graph fused lasso solver that best suits the target graph structure. 



Despite being a popular algorithm for many constrained optimization problems, the convergence of ADMM does not have a simple and unified answer. We present the convergence of Algorithm~\ref{alg:palm} in the following theorem. 
\begin{theorem}
Algorithm~\ref{alg:palm} converges linearly to the unique global optimum of problem~\eqref{eq:cons_opt}.
\label{thm:admm_converge}
\end{theorem}
To obtain the result, we first convert problem~\ref{eq:cons_opt} into a two-block problem; then apply recent result in general two-block problems~\cite{nishihara2015general} to complete the proof. The detailed proof is deferred to supplementary materials.

\subsection{Software}
We provide the open source python code for implementation of Algorithm~\ref{alg:palm} on github (the link is removed in the double blinded version). % \url{https://github.com/summeryingliu/imagereg}.
